Tight Last-Iterate Convergence of the Extragradient and the Optimistic Gradient Descent-Ascent Algorithm for Constrained Monotone Variational Inequalities

The monotone variational inequality is a central problem in mathematical programming that unifies and generalizes many important settings such as smooth convex optimization, two-player zero-sum games, convex-concave saddle point problems, etc. The extragradient algorithm by Korpelevich [1976] and the optimistic gradient descent-ascent algorithm by Popov [1980] are arguably the two most classical and popular methods for solving monotone variational inequalities. Despite their long histories, the following major problem remains open. What is the last-iterate convergence rate of the extragradient algorithm or the optimistic gradient descent-ascent algorithm for monotone and Lipschitz variational inequalities with constraints? We resolve this open problem by showing that both the extragradient algorithm and the optimistic gradient descent-ascent algorithm have a tight $O\left(\frac{1}{\sqrt{T}}\right)$ last-iterate convergence rate for arbitrary convex feasible sets, which matches the lower bound by Golowich et al. [2020a,b]. Our rate is measured in terms of the standard gap function. At the core of our results lies a non-standard performance measure -- the tangent residual, which can be viewed as an adaptation of the norm of the operator that takes the local constraints into account. We use the tangent residual (or a slight variation of the tangent residual) as the the potential function in our analysis of the extragradient algorithm (or the optimistic gradient descent-ascent algorithm) and prove that it is non-increasing between two consecutive iterates.

==> COLT/conclusion.tex <==
\section{Conclusion}~\label{sec:conclusion}
We propose a new method based on SOS programming to analyze iterative algorithms. Combining with the low-dimensionality of the EG and OGDA update rules, we provide the first and tight last-iterate convergence rate of the EG and ODGA algorithm for constrained monotone and Lipschitzs VIs, which, to the best of our knowledge, is also the first last-iterate convergence rate for any p-SCLI algorithm in the constrained setting. We believe many other  iterative methods also have the low-dimensionality that make them amenable to our SOS programming based analysis. %We use the projected Hamiltonian in our paper to measure convergence. Indeed, the SOS programming approach has the flexibility to also search for a function to measure convergence, as long as we provide it with a set of ``basis'' functions. We derive our analysis for the proximal point method using this extra flexibility.
